AWD3: Dynamic Reduction of the Estimation Bias

Value-based deep Reinforcement Learning (RL) algorithms suffer from the estimation bias primarily caused by function approximation and temporal difference (TD) learning. This problem induces faulty state-action value estimates and therefore harms the performance and robustness of the learning algorithms. Although several techniques were proposed to tackle, learning algorithms still suffer from this bias. Here, we introduce a technique that eliminates the estimation bias in off-policy continuous control algorithms using the experience replay mechanism. We adaptively learn the weighting hyper-parameter beta in the Weighted Twin Delayed Deep Deterministic Policy Gradient algorithm. Our method is named Adaptive-WD3 (AWD3). We show through continuous control environments of OpenAI gym that our algorithm matches or outperforms the state-of-the-art off-policy policy gradient learning algorithms.

==> redundant.tex <==
\textbf{Theorem} \textit{Assume we have 2 value estimators $Q_i$ for $i=1,2$ and $Q^*$ indicates the true state action value.} Let the estimate errors $\epsilon_i=Q_i(s,a)-Q^*(s,a)$ be independently identically distributed $ \epsilon_i \sim \mathcal{N}(0,\sigma^2)$. If we take $Q_3 = min\{Q_1, Q_2\}$ as target for the update then, \\
$$\mathbb{E}[\epsilon_3]=-\sigma\frac{1}{\sqrt{\pi}} $$
where $\epsilon_3=Q_3(s,a)-Q^*(s,a)$

\textbf{Proof}
$$\mathbb{E}[\epsilon_3]=\mathbb{E}[\min_{i=1,2}\{Q_i\}-Q^*]=\mathbb{E}[\min_{i=1,2}\{\epsilon_i\}]$$

We can decompose $min\{\epsilon_1, \epsilon_2\}\ $ as  $\frac{1}{2}(\epsilon_1+\epsilon_2-|\epsilon_1-\epsilon_2|)$. The expected value of $\epsilon_1$ and $\epsilon_2$ is 0. 

$$\mathbb{E}[min\{\epsilon_1, \epsilon_2\}]=\frac{1}{2}\mathbb{E}[|\epsilon_1-\epsilon_2|]$$

Let $u=-|\epsilon_1-\epsilon_2|$ then we know $u \sim \mathcal{N}(0,\sigma^2)$

\begin{equation}
\begin{aligned}
\mathbb{E}[u] &= - \int_{-\infty}^{\infty}\frac{1}{\sqrt{2\pi\cdot2\sigma^2}}|u|\exp\{-\frac{u^2}{2\cdot2\sigma^2}\}du  \\
&= -\frac{2}{\sqrt{4\pi\sigma^2}}\int_{0}^{\infty}u\exp\{-\frac{u^2}{4\sigma^2}\} du = -\frac{2\sigma}{\sqrt{\pi}}
\end{aligned}
\end{equation}

\textbf{Theorem}

Assume value function estimator perfectly approximate the true Q values, in expectation over the steady-state distribution.

\begin{equation}
\begin{aligned}
\begin{array}{l}
\mathbb{E}_{s \sim \pi}\left[Q_{\theta}\left(s, \pi_{\text {new }}(s)\right)\right]=\mathbb{E}_{s \sim \pi}\left[Q^{\pi}\left(s, \pi_{\text {new }}(s)\right)\right] \\
\forall \phi_{\text {new }} \in\left[\phi, \phi+\beta\left(\phi_{\text {true }}-\phi\right)\right] \text { such that } \beta>0
\end{array}
\end{aligned}    
\end{equation}

\textbf{Proof}

\subsection{Triplet Delayed Deep Deterministic Policy Gradient (TCD3)}

Recent work on the underestimation bias in continuous state-action space is deeply observed in \textbf{cite triplet}. The authors employed three critics to construct an update function for the computation of target Q-value. The label is provided as follows:

\begin{equation}
    y \leftarrow r + \gamma \mathrm{min} \left(  {\mathrm{max}}(Q_{\theta'_{1}}(s', \tilde{a}), Q_{\theta'_{2}}(s', \tilde{a})), Q_{\theta'_{3}}(s', \tilde{a})\right)
\end{equation}

The authors demonstrated the underestimation bias in TD3 algorithm without assuming that the two critic networks are independent random variables. Therefore, their theoretical approach to reveal the underestimation in continuous state-action spaces is more accurate. This approach aims to further reduce the estimation bias in the face of computational burden. The results have shown that critics trained using this mechanism has more accurate Q value estimations \textbf{cite triplet}.  

\begin{algorithm}
\caption{UpdateBeta} 
\begin{algorithmic}   
\STATE \textbf{Input} $B\textsubscript{beta}, \mu, \beta $
\STATE Sample a batch of $\tilde{N}$ transitions $\left(s, a, r, s^{\prime}\right)$ from $\mathcal{B\textsubscript{beta}}$
\STATE $ \tilde{y} \leftarrow \beta \min _{i=1,2}Q(s,a;\theta_{i}^{\prime}) + \frac{1 - \beta}{2} \sum_{i=1}^{2} Q(s,a;\theta_{i}^{\prime}) $  
\STATE $ \beta \leftarrow \beta - \mu * \tilde{N}^{-1} \sum (r - \tilde{y}) $ 
 
\STATE \textbf{return} $ \beta $  
\end{algorithmic}
\label{alg:alg_beta_update}
\end{algorithm}

\begin{figure}[h]
	\centering
	\subfigure{
		\includegraphics[width=2.5in]{beta values/LunarLanderContinuous-v2_beta.png}}
	\caption{The mean value of $\beta$ throughout the process of training AWD3 agent in LunarLanderContinuous-v2 environment. The shaded area stands for a standard deviation of the average evaluation over 5 random seeds.} 
	\label{beta_change}
\end{figure}
